Deep3DSketch+\+: High-Fidelity 3D Modeling from Single Free-hand Sketches

The rise of AR/VR has led to an increased demand for 3D content. However, the traditional method of creating 3D content using Computer-Aided Design (CAD) is a labor-intensive and skill-demanding process, making it difficult to use for novice users. Sketch-based 3D modeling provides a promising solution by leveraging the intuitive nature of human-computer interaction. However, generating high-quality content that accurately reflects the creator's ideas can be challenging due to the sparsity and ambiguity of sketches. Furthermore, novice users often find it challenging to create accurate drawings from multiple perspectives or follow step-by-step instructions in existing methods. To address this, we introduce a groundbreaking end-to-end approach in our work, enabling 3D modeling from a single free-hand sketch, Deep3DSketch+$\backslash$+. The issue of sparsity and ambiguity using single sketch is resolved in our approach by leveraging the symmetry prior and structural-aware shape discriminator. We conducted comprehensive experiments on diverse datasets, including both synthetic and real data, to validate the efficacy of our approach and demonstrate its state-of-the-art (SOTA) performance. Users are also more satisfied with results generated by our approach according to our user study. We believe our approach has the potential to revolutionize the process of 3D modeling by offering an intuitive and easy-to-use solution for novice users.

==> fig/pic3.tex <==
\vspace{-2em}
\centering
\includegraphics[width=1\linewidth]{fig/pic_3.jpg}
\vspace{-1em}

==> table/table2.tex <==

%% table 2

\begin{table*}[ht]
\begin{center}
\caption{The quantitative evaluation of ShapeNet-Sketch dataset}
\scalebox{0.84}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{15}{|c|}{Shapenet-Sketch (Voxel IoU $\uparrow$)} \\
\hline
& { Cabinet} & { Bench} & { Display} & { Loudspeaker} & { Telephone} & { Rifile} & { Watercraft} & { Lamp} & { Airplane} & { Sofa} & { Table} & { Chair} & { Car} & mean           \\ \hline

Retrieval    & 0.431    & 0.219        & 0.338     & 0.365        & 0.536         & 0.413          & 0.369      & 0.223       & 0.411        & 0.431         & 0.232             & 0.238     & 0.626         & 0.370          \\ \hline

Auto-Encoder       & 0.534       & 0.347        & 0.472    & 0.533       & 0.537          & 0.541           & 0.456             & 0.328             & 0.469             & 0.534     & 0.359       & 0.361       & 0.648        & 0.372          \\ \hline
sketch2model                & \textbf{0.568}                 & 0.366                        & \textbf{0.479}                 & \textbf{0.544}                     & 0.554                            & 0.534                         & 0.466                             & 0.338                       & 0.487                           & \textbf{0.534}                       & 0.357                        & \textbf{0.393}               & 0.659                      & 0.483          \\ \hline

{ Ours} & 0.551                          & \textbf{0.374}               & 0.456                          & 0.503                              &\textbf{0.557}                            & \textbf{0.553}                & \textbf{0.473}                    & \textbf{0.339}                       & \textbf{0.489}                           & 0.533                       & \textbf{0.381}               & 0.389                        & \textbf{0.695}             & \textbf{0.484} \\
\hline
\end{tabular}}

\end{center}

\label{table:table2}

\end{table*}

%
%deep3dsketch+               & 0.553                          & 0.368                        & 0.463                          & 0.514                              & \textbf{0.576}                   & 0.543                         & 0.467                             & \textbf{0.347}              & \textbf{0.490}                  & \textbf{0.534}              & 0.370                        & 0.382                        & 0.675                      & 0.483          \\ \hline
%
